Optimal Algorithms for Augmented Testing of Discrete Distributions

We consider the problem of hypothesis testing for discrete distributions. In the standard model, where we have sample access to an underlying distribution $p$, extensive research has established optimal bounds for uniformity testing, identity testing (goodness of fit), and closeness testing (equivalence or two-sample testing). We explore these problems in a setting where a predicted data distribution, possibly derived from historical data or predictive machine learning models, is available. We demonstrate that such a predictor can indeed reduce the number of samples required for all three property testing tasks. The reduction in sample complexity depends directly on the predictor's quality, measured by its total variation distance from $p$. A key advantage of our algorithms is their adaptability to the precision of the prediction. Specifically, our algorithms can self-adjust their sample complexity based on the accuracy of the available prediction, operating without any prior knowledge of the estimation's accuracy (i.e. they are consistent). Additionally, we never use more samples than the standard approaches require, even if the predictions provide no meaningful information (i.e. they are also robust). We provide lower bounds to indicate that the improvements in sample complexity achieved by our algorithms are information-theoretically optimal. Furthermore, experimental results show that the performance of our algorithms on real data significantly exceeds our worst-case guarantees for sample complexity, demonstrating the practicality of our approach.

==> ack.tex <==
\section*{Acknowledgments}
Part of this work was conducted while the authors were visiting the Simons Institute for the Theory of Computing.
M.A. was supported by NSF awards CNS-2120667, CNS-2120603, CCF-1934846, and BU’s Hariri Institute for Computing. This work was initiated while M.A. was affiliated with Boston University and Northeastern University and was done in part while M.A. was a research fellow at the Simons Institute for the Theory of Computing. P.I. was supported by the NSF TRIPODS program (award DMS-2022448) and Simons Investigator Award.
R.R. was supported by the NSF TRIPODS program (award DMS-2022448) and CCF-2310818.

==> closeness_UB_short_version.tex <==
\section{Upper bound for closeness testing}\label{sec:UB_closeness_short}

Our upper bound is inspired by the \emph{flattening} technique, previously proposed by Diakonikolas and Kane~\cite{DiakonikolasK16}. This technique reduces the $\ell_2$-norm of the underlying distribution, ultimately decreasing the sample complexity of closeness testing. We adapt this technique for use in the augmented setting, aiming not only to flatten the distribution based on received samples but also to exploit the prediction distribution $\hat{p}$. We demonstrate that augmented flattening can significantly reduce the $\ell_2^2$-norm of $p$.

\paragraph{Background on flattening:}
Suppose we are given $n$ parameters $m_1, m_2, \ldots, m_n$. We can create a randomized mapping $F$ that assigns each $i \in [n]$ to a pair $(i,j)$, where $j$ is drawn uniformly at random from $[m_i]$. Consider a distribution $\p$ over $[n]$ and a sample $i$ drawn from $\p$. This mapping induces a distribution over the pairs $(i,j)$ in 
$D \coloneqq \{(i,j) | i \in [n] \mbox{ and } j \in [m_i]\}.$
We denote this new distribution by $\pF$, satisfying the relation:
$\pF_{(i,j)} = \p_i/m_i.$
The core idea of this mapping is to divide the probability of the $i$-th element into $m_i$ {\em buckets}. If the values of $m_i$ are large for elements in $\p$ with higher probabilities, then the resulting distribution $\pF$ avoids having elements with disproportionately large probabilities, thereby naturally reducing its $\ell_2$-norm.



\paragraph{Augmented flattening}
In the following lemma, we propose a new flattening scheme that determines $m_i$'s based on both samples from $\p$ and the prediction $\hp$. We show that if $\hp$ is $\alpha$-close to $\p$, the augmented flattening reduces the $\ell_2^2$-norm of $\p$ so that it becomes linear in $\alpha$. This observation is a key to the resilience of our algorithm to inaccurate predictions: After the flattening step, we can verify whether the $\ell_2^2$-norm of $p$ has indeed dropped to the desired value. If not, then the algorithm concludes that $\hat{p}$ was not $\alpha$-close, and hence, outputting \inaccurate. Otherwise, if the $\ell_2^2$-norm of $p$ is sufficiently small, we proceed with an efficient testing algorithm that requires fewer samples, proportional to the new $\ell_2^2$-norm of $p$.

\begin{lemma}\label{lem:l2norm_bound}
	Suppose we have an unknown distribution $p = (p_1, p_2, \ldots, p_n)$ over $[n]$ and $\poi(\sf)$ samples from $p$. Assume we are given a known distribution $\hp$ that is $\alpha$-close to $\p$ in TV distance. Then for every $v \leq 1$, there exists a flattening $F$ which increases the domain size by $1/v + \sf$ in expectation, and the expected $\ell_2^2$-norm of the $\pF$ is bounded by: $
	\E{\lTwo{\pF}^2} \leq  \frac{2\alpha}{\sf} + 4\cdot \nu.$
The expectation above is taken over the randomness of the samples from $\p$.
\end{lemma}
\begin{proof}
Let $\hatsf \coloneqq \poi(\sf)$ be a Poisson random variable with mean $\sf$.
Let $\F$ denote the multiset of $\hatsf$ samples from $\p$. Let $f_i$ denote the frequency of element $i$ in $\F$. 
For every $i$, we define the number of buckets for element $i$ as follows: 
\begin{equation}
\label{eq:mi_def}
m_i \coloneqq \floor{\frac{\hp_i}{\nu}} + f_i + 1\,.
\end{equation}
Let $\pF$ denote the flattened version of $\p$ where we split every element $i$ into $m_i$ buckets. We show that the expected $\ell_2$-norm of $\pF$ is low. Define $\Delta_i$ to be $\p_i - \hp_i$. Suppose $A$ is a set of indices $i \in [n]$ for which $\Delta_i \geq \hp_i$.  For every $i \in A$, $\p_i$ is bounded from above by $2\,\Delta_i$. On the other hand, for every $i \in [n]\setminus A$, $p_i$ is bounded by $2\,\hp_i$. 

\begin{align*}
	\lTwo{\pF}^2 
	&
	= \sum_{i\in[n]}\sum_{j \in [m_i]} \pF(i,j)^2 
	= \sum_{i\in[n]} \frac{\p_i^2}{m_i} 
	= \sum_{i \in A} \frac{2\,\Delta_i \cdot p_i}{m_i}
    + 
    \sum_{i\in[n]\setminus A} \frac{(2\,\hp_i)^2}{m_i}
    \\ & \leq 
	\sum_{i \in A} \frac{2\,\Delta_i \cdot p_i}{f_i + 1}
	+ 
	\sum_{i\in[n]\setminus A} \frac{(2\,\hp_i)^2}{\hp_i/\nu} 
	%\\ & 
 \leq \sum_{i \in A} \frac{2\,\Delta_i \cdot p_i}{f_i + 1}
	+ 4\,\nu. 
\end{align*}
%The last equality above is due to the fact that for the elements in $A$, $\p_i/2$ is at least $\hp_i$, so $\Delta_i$ is at least $\p_i/2$.
As shown in~\cite{DiakonikolasK16}, the expected value of $\p_i/(f_i + 1)$ taken over the randomness in the samples is bounded by $1/\sf$:
$\E[F]{\p_i/(f_i + 1)} \leq \frac{1}{\sf}$.
Therefore, we obtain: $\E[F]{\lTwo{\pF}^2} \leq \sum_{i \in A} \frac{2\,\Delta_i}{\sf} + 4\,\nu \leq \frac{2\,\alpha}{\sf} + 4\,\nu\,$.


The last inequality above is due to the fact that: 
$\sum_{i\in A} \Delta_i = \p(A) - \hp(A) \leq \tv{p - \hp} = \alpha\,$.
\end{proof}


\paragraph{The algorithm:} 
We provide an algorithm for testing the closeness of two distributions in the augmented setting using the augmented flattening step. Our algorithm receives a suggested accuracy level $\alpha$. Based on $\alpha$, we draw $\sf$ (which depends on $\alpha$) samples from $\p$ and use them to flatten $\p$. 
Next, we check if the $\ell_2^2$-norm of $p$ is reduced after flattening to the desired bound. If not, this indicates that the prediction was not sufficiently accurate, leading us to output \inaccurate. Conversely, if the $\ell_2^2$-norm of $p$ is small, we proceed with a standard  efficient testing algorithm that requires a number of samples proportionate to this lowered $\ell_2^2$-norm.
The pseudocode of our algorithm is provided in Algorithm~\ref{alg:closeness_with_alpha}, and we prove its performance in Theorem~\ref{thm:closeness_with_alpha}.


\begin{algorithm}[ht]
\caption{An augmented tester for testing closeness of $\p$ and $\q$ with a suggested value $\alpha$}
\label{alg:closeness_with_alpha}
\begin{algorithmic}[1]
\Procedure{\textproc{Augmented-Closeness-Tester}}{$n,\ \alpha,\ \epsilon,\ \delta = 2/3,\ \hp$,  sample access to $\p$ and $\q$}
\State{$\sf  \gets  \min\left(n^{2/3} \alpha^{1/3}/\epsilon^{4/3}, n\right)$}
\State{$\hatsf \gets \poi(\sf)$}
\If{$\hatsf > 100\,\sf$}
\State{\Return \reject.}\label{line:closeness_large_poi}
\EndIf
%\State{Draw $\hatsf \coloneqq \poi(\sf)$ samples from $\p$.}
\State{$F \gets F(m_1, m_2, \ldots, m_n)$ where $m_i$ are defined in Equation~\ref{eq:mi_def_alg}.}
\State{$L_p \gets$ \textsc{Estimate-$\ell_2^2$} $\left(\pF,\ \sum_{i=1}^n m_i,\ 0.05 \right)$}
\State{$L_q \gets$ \textsc {Estimate-$\ell_2^2$} $\left(\qF,\ \sum_{i=1}^n m_i,\ 0.05 \right)$}
\If {$L_p > 30\left(\frac{2\alpha}{\sf} + \frac{4}{n}\right)$}
\State{\Return \inaccurate.}\label{line:closeness_output_inaccurate}
\Else \If {$L_q > 90\left(\frac{2\alpha}{\sf} + \frac{4}{n}\right)$}
\State{\Return \reject.}\label{line:closeness_reject}
\Else
\State{\Return \textsc{Closeness-Tester} $\left(\epsilon,\ \delta = 0.01,\ b = 90\left(\frac{2\alpha}{\sf} + \frac{4}{n}\right),\ \pF,\ \qF\right)$.}\label{line:closeness_standard_tester}
\EndIf
\EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}



\begin{theorem}\label{thm:closeness_with_alpha}
For any given parameters $n,\ \alpha,\ \epsilon$, and any two unknown distributions $\p$ and $\q$ and a known predicted distribution $\hp$ for $\p$, Algorithm~\ref{alg:closeness_with_alpha} is an $(\alpha,\ \epsilon,\delta = 0.3)$-augmented tester for testing closeness of $p$ and $q$, which uses $O(n^{2/3}\alpha^{1/3}/\epsilon^{4/3})$ samples. 
\end{theorem}
\begin{proof} We begin the proof by setting our parameters. 
Set $\sf \coloneqq \min\left(n^{2/3} \alpha^{1/3}/\epsilon^{4/3}, n\right)$. Suppose we draw  $\hatsf = \poi(\sf)$ samples from $\p$. We flatten the distribution $\p$ according to the augmented flattening described 
earlier, replacing $\nu$ with $1/n$. We denote the flattening by $F = F(m_1, \ldots, m_n)$ where $m_i$'s are defined in Equation~\eqref{eq:mi_def}: 
\begin{equation}\label{eq:mi_def_alg}
    m_i \coloneqq \floor{n \cdot \hp_i} + f_i + 1\,.
\end{equation}
In the above definition, $f_i$ is the frequency of element $i$ among the $\hatsf$ drawn samples.


\paragraph{Proof of correctness:} Suppose we  flatten both $\p$ and $\q$ according to $F$. The algorithm estimates the $\ell_2^2$ of $\pF$ and $\qF$. According to Fact~\ref{fct:ell2_estimation}, these estimates are within a constant factor of their true values each with probability at least $1-0.05$:
\begin{equation}
\label{eq:Lpq22Bounds}
\frac{\lTwo{\pF}}{2} \leq L_p \leq \frac{3\,\lTwo{\pF}}{2}\, \quaad \text{and} \quaad \frac{\lTwo{\qF}}{2} \leq L_q \leq \frac{3\,\lTwo{\qF}}{2}\,.
\end{equation}
To prove the correctness of the algorithm, we show the three desired property of an augmented tester which are defined in Definition~\ref{def:AugmentedTester}. First, assume $\hp$ is $\alpha$-close to $\p$. We show the probability of outputting \inaccurate is small. Using Lemma~\ref{lem:l2norm_bound}, after applying $F$,  the expected $\ell_2^2$-norm of $\pF$ is bounded by: $
    \E{\lTwo{\pF}} \leq \frac{2\alpha}{\sf} + \frac{4}{n} %\leq \max \left( \frac{2\,\alpha^{2/3} \cdot \epsilon^{4/3}}{n^{2/3}} + \frac{4}{n},\ \frac{6}{n}\right)
    \,.$
Using Markov's inequality, with probability at least 0.95, $\ell_2^2$-norm of $\pF$ is at most 20 times the above bound.
Combined with the upper bound for $L_p$ in Equation~\eqref{eq:Lpq22Bounds} and the union bound, in this case $L_p$ is bounded by $30 \cdot \left(2\alpha/\sf + 4/n\right)$ with probability at least 0.9. Hence, the algorithm does not output \inaccurate in Line~\ref{line:closeness_output_inaccurate} with probability more than 0.1. 

Next, we show that if $p = q$, the algorithm outputs \reject with a small probability. 
We may output \reject in three cases: 1) in Line~\ref{line:closeness_large_poi} 2) in Line~\ref{line:closeness_reject} and 3) in Line~\ref{line:closeness_standard_tester}. Using Markov's inequality, a Poisson random variable exceeds 100 times its expectation with probability at most 0.01. We show the other two cases are unlikely as long as $L_p$ and $L_q$ are accurate estimates of the $\ell_2^2$s of $\pF$ and $\qF$ (which happens with probability of 0.9). 
If $\p = \q$, $\pF$ and $\qF$ are identical. Therefore, in the algorithm, $L_p$ and $L_q$ are the estimations of the $\ell_2^2$-norm of the same distribution.
Note that we output \reject in Line~\ref{line:closeness_reject}, only when $L_p < 3 L_q$. Using Equation~\eqref{eq:Lpq22Bounds}, this event does not happen unless at least one of the estimates is inaccurate (which has a probability at most 0.1).
Furthermore, if the estimated $\ell_2^2$-norms are accurate, the minimum $\ell_2^2$-norms of $\pF$ and $\qF$ are bounded by $90 \cdot \left(2\alpha/\sf + 4/n\right)$, implying the tester would work correctly with probability at least 0.99. Using the union bound, the probability of outputting \reject is bounded by 0.12. 



Finally, we show that if $\p$ is $\epsilon$-far from $\qF$, the probability of outputting \accept is small. We only output \accept in Line~\ref{line:closeness_standard_tester}. Similar to the second case we have discussed, as long as the $\ell_2^2$-norms are accurate, the tester does not make a mistake with a probability more than 0.01. Therefore, the overall probability of making a mistake is bounded by 0.11. 

%\textcolor{red}{we should have a theorem statement about Closeness-Tester that we reference in the proof.}
%\ma{Yes, That is Fact~\ref{fct:standard_closeness} we use below}



\paragraph{Analysis of sample complexity:} For the flattening step, we have used $\hatsf \leq 10 \sf$. After flattening, the new domain size is bounded from above by: 
$\sum_{i=1}^n m_i \leq \sum_{i=1}^n n \cdot \hp_i + f_i + 1 = n + \hatsf + n \leq 12n.$
Using Fact~\ref{fct:ell2_estimation}, estimation of $\ell_2^2$-norm requires $O(\sqrt{n})$ samples. 
Using Fact~\ref{fct:standard_closeness}, the number of samples we use for the test in Line~\ref{line:closeness_standard_tester} is $O(n\cdot b/\epsilon^2)$ samples. Hence, the total sample complexity is:

\begin{align*}
	\text{\# samples} & = O \left( \sf + \sqrt{n} + 
	\frac{n \cdot b}{\epsilon^2} 
	\right) = O\left( \sf + \sqrt{n} + 
	\frac{n\cdot\sqrt{2\alpha/\sf + 4/n} }{\epsilon^2}
	\right)
	 \\ & 
  =  O\left(
        \frac{\sqrt{n}}{\epsilon^2} + \frac{n^{2/3}\,\alpha^{1/3}}{\epsilon^{4/3}}\right)
	 \,.
\end{align*}
In the last line, we use that $\sf \coloneqq \min\left(n^{2/3} \alpha^{1/3}/\epsilon^{4/3}, n\right)$. Thus, the proof is complete.
\end{proof}




%\textcolor{red}{sandeep: i checked up to here. will continue later}
% ma: thank you!


